AutoAD II: The Sequel -- Who, When, and What in Movie Audio Description

Audio Description (AD) is the task of generating descriptions of visual content, at suitable time intervals, for the benefit of visually impaired audiences. For movies, this presents notable challenges -- AD must occur only during existing pauses in dialogue, should refer to characters by name, and ought to aid understanding of the storyline as a whole. To this end, we develop a new model for automatically generating movie AD, given CLIP visual features of the frames, the cast list, and the temporal locations of the speech; addressing all three of the 'who', 'when', and 'what' questions: (i) who -- we introduce a character bank consisting of the character's name, the actor that played the part, and a CLIP feature of their face, for the principal cast of each movie, and demonstrate how this can be used to improve naming in the generated AD; (ii) when -- we investigate several models for determining whether an AD should be generated for a time interval or not, based on the visual content of the interval and its neighbours; and (iii) what -- we implement a new vision-language model for this task, that can ingest the proposals from the character bank, whilst conditioning on the visual features using cross-attention, and demonstrate how this improves over previous architectures for AD text generation in an apples-to-apples comparison.

==> figures/arch_code.tex <==
\newcommand\algcomment[1]{\def\@algcomment{\footnotesize#1}}
\begin{algorithm}[h]
	\caption{PyTorch Code for the AD generation model.}\label{code}
	\begin{lstlisting}[language=python]
import torch
import torch.nn as nn
from transformers.models.gpt2 import GPT2Attention, GPT2MLP, GPT2Block
from einops import rearrange
from typing import Tuple, Union, Optional
from collections import OrderedDict

class QuickGELU(nn.Module):
    def forward(self, x: torch.Tensor):
        return x * torch.sigmoid(1.702 * x)

class PerceiverResampler_Step(nn.Module):
    def __init__(self, d_model: int, n_head: int,):
        super().__init__()
        self.attn = nn.MultiheadAttention(d_model, n_head)
        self.ln_1 = nn.LayerNorm(d_model)
        self.mlp = nn.Sequential(OrderedDict([
            ("c_fc", nn.Linear(d_model, d_model * 4)),
            ("gelu", QuickGELU()),
            ("c_proj", nn.Linear(d_model * 4, d_model))
        ]))
        self.ln_2 = nn.LayerNorm(d_model)

    def with_pos_embed(self, tensor, pos: Optional[torch.Tensor]):
        raise NotImplementedError
        return tensor if pos is None else tensor + pos

    def attention(self, x: torch.Tensor, kv: torch.Tensor, key_padding_mask: torch.Tensor = None):
        key_padding_mask = key_padding_mask.to(device=x.device) if key_padding_mask is not None else None
        return self.attn(x, kv, kv, need_weights=False, key_padding_mask=key_padding_mask)[0]

    def forward(self, x: torch.Tensor, kv: torch.Tensor, key_padding_mask: torch.Tensor = None):
        """q=x, kv=concat([x_f, x])"""
        x_norm = self.ln_1(x)
        x = x + self.attention(x_norm, kv, key_padding_mask=key_padding_mask)
        x = x + self.mlp(self.ln_2(x))
        return x, x_norm


class PerceiverResampler_Blocks(nn.Module):
    """the official perceiver resampler in Flamingo:
    for i in range(num_layers):
        x = x + attention_i(q=x, kv=concat([x_f, x]))
        x = x + ffw_i(x)
    return x
    """
    def __init__(self, width: int, layers: int, heads: int,):
        super().__init__()
        self.width = width
        self.layers = layers
        self.resblocks = nn.ModuleList([PerceiverResampler_Step(width, heads) for _ in range(layers)])

    def forward(self, x: torch.Tensor, visual: torch.Tensor, key_padding_mask: torch.Tensor = None):
        intermediate = []
        for block in self.resblocks:
            kv = torch.cat((x, visual), dim=0)  # x,B,C
            x, x_norm = block(x=x, kv=kv, key_padding_mask=key_padding_mask)
            intermediate.append(x_norm)
        intermediate.pop(0)
        intermediate.append(x)  # the last one is NOT normed
        return intermediate
    

class PerceiverResampler(nn.Module):
    """the official perceiver resampler in Flamingo:
    x_f = x_f + time_embeddings
    x_f = flatten(x_f)
    for i in range(num_layers):
        x = x + attention_i(q=x, kv=concat([x_f, x]))
        x = x + ffw_i(x)
    return x
    """
    def __init__(self, num_latents=16, d_latents=768, nhead=8, num_layers=2, num_hypo=1):
        super().__init__()
        assert num_hypo == 1
        # TODO: implement MH
        self.num_latents = num_latents
        self.latent = nn.Parameter(torch.empty(num_latents * num_hypo, d_latents))
        self.temporal_pos_embed = nn.Parameter(torch.empty(512, d_latents))
        self.encoder = PerceiverResampler_Blocks(width=d_latents, layers=num_layers, heads=nhead)
        self.visual_prenorm = nn.LayerNorm(d_latents)
        self.initialize_parameters()

    def initialize_parameters(self):
        nn.init.normal_(self.latent, mean=0, std=1)
        nn.init.normal_(self.temporal_pos_embed, mean=0, std=1.0)
        # init decoder
        proj_std = (self.encoder.width ** -0.5) * ((2 * self.encoder.layers) ** -0.5)
        attn_std = self.encoder.width ** -0.5
        fc_std = (2 * self.encoder.width) ** -0.5
        for block in self.encoder.resblocks:
            nn.init.normal_(block.attn.in_proj_weight, std=attn_std)
            nn.init.normal_(block.attn.out_proj.weight, std=proj_std)
            nn.init.normal_(block.mlp.c_fc.weight, std=fc_std)
            nn.init.normal_(block.mlp.c_proj.weight, std=proj_std)

    def forward(self, visual_feature, key_padding_mask=None):
        B, T, *_ = visual_feature.shape
        visual_feature = rearrange(visual_feature, 'b t c -> t b c')
        temp_pos = self.temporal_pos_embed[0:T, None, :]
        visual_feature = self.visual_prenorm(visual_feature) + temp_pos
        latent = self.latent[:,None,:].repeat(1,B,1)  # k,b,c
        latent_out = self.encoder(x=latent, 
                                  visual=visual_feature, 
                                  key_padding_mask=key_padding_mask)[-1]  # last layer output
        return rearrange(latent_out, 'k b c -> b k c')
    

class GPT2Block_GatedXATTN(nn.Module):
    """Patch the implementation of GPT2Block from HuggingFace by inserting a Gated XATTN block"""
    def __init__(self, config, layer_idx=None):
        super().__init__()
        hidden_size = config.hidden_size
        inner_dim = config.n_inner if config.n_inner is not None else 4 * hidden_size

        self.ln_1 = nn.LayerNorm(hidden_size, eps=config.layer_norm_epsilon)
        self.attn = GPT2Attention(config, layer_idx=layer_idx)
        self.ln_2 = nn.LayerNorm(hidden_size, eps=config.layer_norm_epsilon)

        ### Gated-XAttn Block ###
        self.xattn_attn = GPT2Attention(config, is_cross_attention=True, layer_idx=layer_idx)
        self.xattn_mlp = GPT2MLP(inner_dim, config)
        self.xattn_attn_gate = nn.Parameter(torch.tensor([0.]))
        self.xattn_ff_gate = nn.Parameter(torch.tensor([0.]))
        ### Gated-XAttn Block ###

        if config.add_cross_attention:
            self.crossattention = GPT2Attention(config, is_cross_attention=True, layer_idx=layer_idx)
            self.ln_cross_attn = nn.LayerNorm(hidden_size, eps=config.layer_norm_epsilon)

        self.mlp = GPT2MLP(inner_dim, config)

    def forward(
        self,
        hidden_states: Optional[Tuple[torch.FloatTensor]],
        layer_past: Optional[Tuple[torch.Tensor]] = None,
        attention_mask: Optional[torch.FloatTensor] = None,
        head_mask: Optional[torch.FloatTensor] = None,
        encoder_hidden_states: Optional[torch.Tensor] = None,
        encoder_attention_mask: Optional[torch.FloatTensor] = None,
        use_cache: Optional[bool] = False,
        output_attentions: Optional[bool] = False,
        media: Optional[torch.FloatTensor] = None,
        media_mask: Optional[torch.FloatTensor] = None,
    ) -> Union[Tuple[torch.Tensor], Optional[Tuple[torch.Tensor, Tuple[torch.FloatTensor, ...]]]]:
        residual = hidden_states
        hidden_states = self.ln_1(hidden_states)

        ### Gated-XAttn starts ###
        if media is not None:
            # hidden_states = hidden_states + (self.xattn_attn_gate) * \
            hidden_states = hidden_states + torch.tanh(self.xattn_attn_gate) * \
                self.xattn_attn(hidden_states,
                    attention_mask=attention_mask,
                    head_mask=head_mask,
                    encoder_hidden_states=media,
                    encoder_attention_mask=media_mask,
                    output_attentions=output_attentions,)[0]
            # hidden_states = hidden_states + (self.xattn_ff_gate) * \
            hidden_states = hidden_states + torch.tanh(self.xattn_ff_gate) * \
                self.xattn_mlp(hidden_states)
        ### Gated-XAttn ends ###

        attn_outputs = self.attn(
            hidden_states,
            layer_past=layer_past,
            attention_mask=attention_mask,
            head_mask=head_mask,
            use_cache=use_cache,
            output_attentions=output_attentions,
        )
        attn_output = attn_outputs[0]  # output_attn: a, present, (attentions)
        outputs = attn_outputs[1:]
        # residual connection
        hidden_states = attn_output + residual

        if encoder_hidden_states is not None:
            # add one self-attention block for cross-attention
            if not hasattr(self, "crossattention"):
                raise ValueError(
                    f"If `encoder_hidden_states` are passed, {self} has to be instantiated with "
                    "cross-attention layers by setting `config.add_cross_attention=True`"
                )
            residual = hidden_states
            hidden_states = self.ln_cross_attn(hidden_states)
            cross_attn_outputs = self.crossattention(
                hidden_states,
                attention_mask=attention_mask,
                head_mask=head_mask,
                encoder_hidden_states=encoder_hidden_states,
                encoder_attention_mask=encoder_attention_mask,
                output_attentions=output_attentions,
            )
            attn_output = cross_attn_outputs[0]
            # residual connection
            hidden_states = residual + attn_output
            outputs = outputs + cross_attn_outputs[2:]  # add cross attentions if we output attention weights

        residual = hidden_states
        hidden_states = self.ln_2(hidden_states)
        feed_forward_hidden_states = self.mlp(hidden_states)
        # residual connection
        hidden_states = residual + feed_forward_hidden_states

        if use_cache:
            outputs = (hidden_states,) + outputs
        else:
            outputs = (hidden_states,) + outputs[1:]

        return outputs  # hidden_states, present, (attentions, cross_attentions)
\end{lstlisting}
\end{algorithm}

==> tables/dataset_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h!]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Statistics of Audio Description datasets.} We report relevant statistics to compare our MAD-v2 and Audiovault datasets.}
\begin{tabular}{@{}lrrrcc@{}}
\toprule
Dataset                        & \begin{tabular}[c]{@{}l@{}}Total \\ movies\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total\\ duration (hrs)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Total AD\\ captions\end{tabular} & Subtitles & \begin{tabular}[c]{@{}l@{}}Visual\\ Features\end{tabular} \\ \midrule

LSMDC~\cite{rohrbach2017movie} & 200                                                     & 147                                                            & 128K                                                        & \xmark   & \cmark                                                    \\
MAD-v1~\cite{soldan2022mad}       & 488                                                     & 892                                                            & 280K                                                        & \cmark    & \cmark                                                    \\
MAD-v2~\cite{han2023auto} & 488                                                     & 892                                                            & 264K                                                        & \cmark    & \cmark                                                    \\
\rowcolor{pastelgray}
AudioVault~\cite{han2023auto}                    & 7,057                                                   & 12,510                                                         & 3.3M                                                        & \cmark    & \xmark
                                                    \\ \midrule
\rowcolor{pastelgray}                                                  
AudioVault-v2 (ours)                    & 7,057                                                   & 12,510                                                         & 3.3M                                                        & \cmark    & \xmark
                                                    \\
MAD-v3 (ours)                    & 488                                                   &                                                   892 & 272K \\
MovieNet-AD (ours)                    & 703                                                   &                                                   1,200 & 600K \\
CMD-AD (ours)                    & 1,600                                                   & 700 & 300K  \\ \midrule
Total visual (ours)                    &2,900                                                   & 2,200 & 1.1M \\

          \bottomrule                                       
\end{tabular}
\label{tab:dataset-compare}
\end{table}

==> tables/finetuning_data.tex <==
\begin{table}
\centering
\caption{\textbf{Effect of data collection pipeline.} We compare the proposed MAD-v3 using the proposed data collection pipeline}
\small
\begin{tabular}{lrrrrr}
\toprule
Finetuning Data      & R-L & C   & S   & BertS \\ \midrule
% {ClipCap~\cite{mokady2021clipcap} & MAD-v2-\texttt{Unnamed} & 8.5 & 4.6 & 3.8 & 16.8  \\
MAD-v1~\cite{mokady2021clipcap} & 12.8 & 17.0 & 5.2 & 21.8  \\
MAD-v2~\cite{mokady2021clipcap} & 13.3 & 17.8 & 5.8 & 22.1 \\
% \multirow{2}{*}{UniVL~\cite{luo2020univl}}        & MAD-v2-\texttt{Unnamed} &     &     &     &       \\
%                                                   & MAD-v2-\texttt{Named}   &     &     &     &       \\
% \midrule
MAD-v3 (ours)   & - & - & - & - \\  \midrule
CMD-AD (ours)   & - & - & - & - \\ 
MovieNet-AD (ours)   & - & - & - & - \\ 
All   & - & - & - & - \\ 
 \bottomrule
\end{tabular}
\label{tab:train-data}
\end{table}

==> tables/mad_cleaning_quant.tex <==
\begin{table}
\scriptsize
\centering
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Effect of denoising MAD training data annotation.} 
We train a model with 6 contextual ADs on MAD-v1~\cite{soldan2022mad}, MAD-v2~\cite{}, and MAD-v3 sources without any pretraining.
The model is evaluated on both the \textbf{\texttt{named}} and \textbf{\texttt{unnamed}} versions of MAD-eval
under the \textbf{oracle} setting.
Cross-domain testing results (when the model is trained and tested on different types of annotations) 
are provided for reference and marked in {\color{gray}gray}.
}
\begin{tabular}{@{}cc|llll|llll@{}}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MAD\\ Train Set\end{tabular}}} & \multicolumn{4}{c}{MAD-eval-\texttt{Unnamed}}   & \multicolumn{4}{c}{MAD-eval-\texttt{Named}}  \\ \cmidrule(l){3-10} 
\multicolumn{2}{c|}{} & \multicolumn{1}{c}{R-L} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{BertS} & \multicolumn{1}{c}{R-L} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{BertS} \\ \midrule
\multirow{2}{*}{v1} & {\texttt{Unnamed}}  & 15.1 & 12.7 & 9.5  & 22.4        & {\color{gray}12.7} & {\color{gray}15.9} & {\color{gray}4.7}  & {\color{gray}22.0}   \\
                    & {\texttt{Named}}    & {\color{gray}11.3} & {\color{gray}10.9} & {\color{gray}3.0}  & {\color{gray}24.0}        & 12.8 & 17.0 & 5.2  & 21.8  \\ \midrule
\multirow{2}{*}{v2} & {\texttt{Unnamed}}  & 15.9 & \textbf{14.5} & \textbf{10.5} & \textbf{26.7}     & {\color{gray}12.9} & {\color{gray}{18.0}} & {\color{gray}4.7} & {\color{gray}22.0} \\
                    & {\texttt{Named}}    & {\color{gray}11.4} & {\color{gray}10.0} & {\color{gray}3.1}  & {\color{gray}22.5}      & \textbf{13.3} & \textbf{17.8}  & \textbf{5.8} & \textbf{22.1} \\ \midrule
\multirow{2}{*}{v3} & {\texttt{Unnamed}}  &  &  &  &  & {\color{gray}} & {\color{gray}{}} & {\color{gray}} & {\color{gray}} \\
                    & {\texttt{Named}}    & {\color{gray}} & {\color{gray}} & {\color{gray}}  & {\color{gray}}      & \textbf{} & \textbf{}  & \textbf{} & \textbf{}     \\ \bottomrule
\end{tabular}
\label{table:cleaning}
\end{table}

